Studying Spectral Behavior, Accretion Processes and Photometric Behavior of Some Binary Stars in the Ultraviolet and Optical Regions

We study the evolution of the normalized flux of selected ultraviolet emission lines of three classical novae (PW Vul, V1668 Cyg and V1974 Cyg). Different phases ofthe outbursts are studied. We attribute the spectral behavior of the three systems to the variation of the optical thickness and temperature of the envelope during the different phases of the outbursts. Our results are consistent with the theoretical models of classical novae. We also present optical photometric observations of the three systems in the post-novae phase. These observations show the variation of the light curves of these systems and the different times of maxima and minima.

==> Makefile <==

PACKAGE=nomencl

SAMPLES = sample01.tex sample02.tex sample03.tex sample04.tex sample05.tex 

CFG = sample04.cfg sample05.cfg sample06.cfg


SAMPLEPDF = ${SAMPLES:%.tex=%.pdf}

PDF = $(PACKAGE).pdf ${SAMPLEPDF}

all:  ${PDF} ${SAMPLES} ${CFG} ${PACKAGE}.sty


%.sty:  %.ins %.dtx
	pdflatex $*.ins

sample%.tex:  nomencl.ins nomencl.sty
	pdflatex nomencl.ins

sample%.cfg: nomencl.ins nomencl.dtx
	pdflatex nomencl.ins


%.pdf:  %.dtx ${PACKAGE}.sty 
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


sample%.pdf: sample%.tex ${CFG} ${PACKAGE}.sty
	pdflatex sample$*.tex
	makeindex sample$*.nlo -s nomencl.ist -o sample$*.nls
	pdflatex sample$*.tex
	pdflatex sample$*.tex



clean:
	$(RM)  ${PACKAGE}.sty *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi *.drv *.ist \
	*.nlo *.nls ${SAMPLES} ${CFG}

distclean: clean
	$(RM) $(PDF) 

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

.PRECIOUS: ${SAMPLES} ${CFG}

